Incorporating Financial Hardship in Measuring the Mental Health Impact of Housing Stress

Housing expenditure tends to be sticky and costly to adjust, and makes up a large proportion of household expenditure. Additionally, the loss of housing can have catastrophic consequences. These specific features of housing expenditure imply that housing stress could cause negative mental health impacts. This research investigates the effects of housing stress on mental health, contributing to the literature by nesting housing stress within a measure of financial hardship, thus improving robustness to omitted variables and creating a natural comparison group for matching. Fixed effects (FE) regressions and a difference-in-differences (DID) methodology are estimated utilising data from the Household Income and Labour Dynamics in Australia (HILDA) Survey. The results show that renters who are in housing stress have a significant decline in self-reported mental health, with those in prior financial hardship being more severely affected. In contrast, there is little to no evidence of housing stress impacting on owners with a mortgage. The results also suggest that the mental health impact of housing stress is more important than some, but not all, aspects of financial hardship.

==> did_results_sum.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Jun 25 17:48:03 2021
\begingroup\normalsize
\begin{tabular}{llrr}
  \hline
Test &  & Renters & Owners \\ 
  \hline
\hline
Parallel Trends & Estimate & 0.13 & -0.21 \\ 
   & p-value & 0.88 & 0.83 \\ 
   \hline
Treatment Effects & Estimate & -2.05 & -0.96 \\ 
   & p-value & 0.02 & 0.31 \\ 
   \hline
\hline
\end{tabular}
\endgroup


==> het_results_rent.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Sat Jun 05 20:20:15 2021
\begin{tabular}{llrrrr}
  &  & $\tau^{(1)}$ & $\tau^{(2)}$ & $\tau^{(3)}$ & F-test \\ 
  \hline
\hline
Renters & Estimate & -1.40 & -1.52 & -1.94 & 0.13 \\ 
   & p-value & 0.08 & 0.15 & 0.01 & 0.88 \\ 
   \hline
Owners & Estimate & 1.00 & 1.00 & 1.00 & 1.00 \\ 
   & p-value & 1.00 & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}


==> het_results_rent_own.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Tue Jun 08 15:00:11 2021
\begingroup\normalsize
\begin{tabular}{llrrrr}
  \hline
Test &  &  Rent: Low & High &  Own: Low & High \\ 
  \hline
\hline
Parallel Trends & Estimate & -0.05 & 0.02 & -0.04 & 0.23 \\ 
   & p-value & 0.95 & 0.97 & 0.93 & 0.74 \\ 
   \hline
Treatment Effects & Estimate & -1.40 & -1.94 & -0.01 & -0.32 \\ 
   & p-value & 0.08 & 0.01 & 0.99 & 0.65 \\ 
   \hline
Equality of & Difference &  & -0.54 &  & -0.31 \\ 
  Treatment Effects  & p-value &  & 0.62 &  & 0.70 \\ 
   \hline
\end{tabular}
\endgroup


==> het_results_rent_own_sens.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Tue Jun 08 16:12:59 2021
\begingroup\normalsize
\begin{tabular}{llrrrr}
  \hline
Test &  &  Rent: Low & High &  Own: Low & High \\ 
  \hline
\hline
Parallel Trends & Estimate & 0.57 & -0.58 & 0.24 & -0.34 \\ 
   & p-value & 0.60 & 0.60 & 0.70 & 0.76 \\ 
   \hline
Treatment Effects & Estimate & -2.08 & -2.69 & -0.05 & -1.39 \\ 
   & p-value & 0.11 & 0.02 & 0.94 & 0.21 \\ 
   \hline
Equality of & Difference &  & -0.61 &  & -1.34 \\ 
  Treatment Effects  & p-value &  & 0.73 &  & 0.31 \\ 
   \hline
\end{tabular}
\endgroup


==> ss_bytenure19.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Summary Statistics By Tenure, 2019}\label{tab.ss.tenure19}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\hline
\hline
Tenure & \multicolumn{3}{c}{Owners} & \multicolumn{3}{c}{Private Renters}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 10538 & 48.6 & 10.57 & 4166 & 44.61 & 12.14 \\ 
Mental health scale & 10728 & 74.27 & 17.1 & 4229 & 68.21 & 19.26 \\ 
Financial hardship & 10550 & 0.13 & 0.33 & 4083 & 0.37 & 0.48 \\ 
Missed housing payments & 10592 & 0.04 & 0.19 & 4119 & 0.11 & 0.31 \\ 
Could not pay bills & 10624 & 0.06 & 0.24 & 4137 & 0.2 & 0.4 \\ 
Sold or pawned something & 10610 & 0.03 & 0.18 & 4124 & 0.12 & 0.33 \\ 
Went without meals & 10615 & 0.02 & 0.14 & 4125 & 0.09 & 0.29 \\ 
Went without heating & 10614 & 0.02 & 0.14 & 4118 & 0.06 & 0.23 \\ 
Sort help from friends or family & 10623 & 0.07 & 0.25 & 4136 & 0.25 & 0.43 \\ 
Sort help from welfare or community organisation & 10608 & 0.02 & 0.13 & 4122 & 0.08 & 0.27 \\ 
Monthly mortgage payments & 6204 & 2096.53 & 1749.82 & 0 & NaN &  \\ 
Monthly rental payments & 0 & NaN &  & 4759 & 1581.09 & 772.29 \\ 
Employed full-time & 11483 & 0.42 & 0.49 & 4762 & 0.49 & 0.5 \\ 
Employed part-time & 11483 & 0.22 & 0.41 & 4762 & 0.21 & 0.41 \\ 
Moved in last 12 months & 11391 & 0.08 & 0.26 & 4744 & 0.37 & 0.48 \\ 
Eqv. household disposable income (\$1,000's) & 11483 & 62.99 & 42.85 & 4762 & 50.41 & 30.7 \\ 
Physical component summary & 10538 & 48.99 & 10.47 & 4166 & 50.56 & 10.43\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> ss_bytenure19a.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Summary Statistics By Tenure, 2019}\label{tab.ss.tenure19}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\hline
\hline
Tenure & \multicolumn{3}{c}{Owners} & \multicolumn{3}{c}{Private Renters}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 10538 & 48.6 & 10.57 & 4166 & 44.61 & 12.14 \\ 
Mental health scale & 10728 & 74.27 & 17.1 & 4229 & 68.21 & 19.26 \\ 
Financial hardship & 10497 & 0.16 & 0.37 & 4052 & 0.44 & 0.5 \\ 
Missed housing payments & 10592 & 0.04 & 0.19 & 4119 & 0.11 & 0.31 \\ 
Could not pay bills & 10624 & 0.06 & 0.24 & 4137 & 0.2 & 0.4 \\ 
Sold or pawned something & 10610 & 0.03 & 0.18 & 4124 & 0.12 & 0.33 \\ 
Went without meals & 10615 & 0.02 & 0.14 & 4125 & 0.09 & 0.29 \\ 
Went without heating & 10614 & 0.02 & 0.14 & 4118 & 0.06 & 0.23 \\ 
Sort help from friends or family & 10623 & 0.07 & 0.25 & 4136 & 0.25 & 0.43 \\ 
Sort help from welfare or community organisation & 10608 & 0.02 & 0.13 & 4122 & 0.08 & 0.27 \\ 
Unable to riase \$2000 (\$3000) for emergency & 10654 & 0.07 & 0.25 & 4162 & 0.21 & 0.4 \\ 
Monthly mortgage payments & 6204 & 2096.53 & 1749.82 & 0 & NaN &  \\ 
Monthly rental payments & 0 & NaN &  & 4759 & 1581.09 & 772.29 \\ 
Employed full-time & 11483 & 0.42 & 0.49 & 4762 & 0.49 & 0.5 \\ 
Employed part-time & 11483 & 0.22 & 0.41 & 4762 & 0.21 & 0.41 \\ 
Neighbourhood decile of disadvantage & 11475 & 5.92 & 2.81 & 4761 & 5.25 & 2.83 \\ 
Eqv. household disposable income (\$1,000's) & 11483 & 62.99 & 42.85 & 4762 & 50.41 & 30.7 \\ 
Physical component summary & 10538 & 48.99 & 10.47 & 4166 & 50.56 & 10.43\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> ss_full0119.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Full Sample Summary Statistics}\label{tab.ss.full0119}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\hline
\hline
Year & \multicolumn{3}{c}{2001} & \multicolumn{3}{c}{2019}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 12323 & 48.59 & 10.4 & 15698 & 47.25 & 11.32 \\ 
Mental health scale & 12933 & 73.72 & 17.48 & 15987 & 72.18 & 18.23 \\ 
Financial hardship & 12574 & 0.29 & 0.45 & 15624 & 0.2 & 0.4 \\ 
Missed housing payments & 12718 & 0.09 & 0.29 & 15707 & 0.06 & 0.23 \\ 
Could not pay bills & 12848 & 0.19 & 0.39 & 15765 & 0.11 & 0.31 \\ 
Sold or pawned something & 12772 & 0.07 & 0.25 & 15733 & 0.06 & 0.24 \\ 
Went without meals & 12783 & 0.05 & 0.21 & 15744 & 0.05 & 0.21 \\ 
Went without heating & 12762 & 0.04 & 0.19 & 15732 & 0.03 & 0.18 \\ 
Sort help from friends or family & 12816 & 0.17 & 0.37 & 15767 & 0.13 & 0.33 \\ 
Sort help from welfare or community organisation & 12787 & 0.05 & 0.23 & 15732 & 0.04 & 0.2 \\ 
Owner & 13969 & 0.72 & 0.45 & 17441 & 0.66 & 0.47 \\ 
Renter & 13969 & 0.26 & 0.44 & 17441 & 0.31 & 0.46 \\ 
Rents from private landlord & 13969 & 0.2 & 0.4 & 17455 & 0.27 & 0.45 \\ 
Rents from public housing & 13969 & 0.04 & 0.2 & 17455 & 0.03 & 0.18 \\ 
Monthly mortgage payments & 4394 & 1502.67 & 1160.26 & 6204 & 2096.53 & 1749.82 \\ 
Monthly rental payments & 3573 & 1050.52 & 565.1 & 5495 & 1490.23 & 838.43 \\ 
Employed full-time & 13969 & 0.42 & 0.49 & 17462 & 0.42 & 0.49 \\ 
Employed part-time & 13969 & 0.2 & 0.4 & 17462 & 0.21 & 0.41 \\ 
Moved in last 12 months & 13957 & 0.19 & 0.39 & 17338 & 0.17 & 0.37 \\ 
Eqv. household disposable income (\$1,000's) & 13969 & 42.44 & 29.82 & 17462 & 57.61 & 39.58 \\ 
Physical component summary & 12323 & 49.68 & 10.5 & 15698 & 49.16 & 10.69\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> ss_full0119a.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Full Sample Summary Statistics}\label{tab.ss.full0119}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\hline
\hline
Year & \multicolumn{3}{c}{2001} & \multicolumn{3}{c}{2019}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 12323 & 48.59 & 10.4 & 15698 & 47.25 & 11.32 \\ 
Mental health scale & 12933 & 73.72 & 17.48 & 15987 & 72.18 & 18.23 \\ 
Financial hardship & 12484 & 0.35 & 0.48 & 15530 & 0.26 & 0.44 \\ 
Missed housing payments & 12718 & 0.09 & 0.29 & 15707 & 0.06 & 0.23 \\ 
Could not pay bills & 12848 & 0.19 & 0.39 & 15765 & 0.11 & 0.31 \\ 
Sold or pawned something & 12772 & 0.07 & 0.25 & 15733 & 0.06 & 0.24 \\ 
Went without meals & 12783 & 0.05 & 0.21 & 15744 & 0.05 & 0.21 \\ 
Went without heating & 12762 & 0.04 & 0.19 & 15732 & 0.03 & 0.18 \\ 
Sort help from friends or family & 12816 & 0.17 & 0.37 & 15767 & 0.13 & 0.33 \\ 
Sort help from welfare or community organisation & 12787 & 0.05 & 0.23 & 15732 & 0.04 & 0.2 \\ 
Unable to riase \$2000 (\$3000) for emergency & 12849 & 0.17 & 0.37 & 15832 & 0.12 & 0.33 \\ 
Owner & 13969 & 0.72 & 0.45 & 17441 & 0.66 & 0.47 \\ 
Renter & 13969 & 0.26 & 0.44 & 17441 & 0.31 & 0.46 \\ 
Rents from private landlord & 13969 & 0.2 & 0.4 & 17455 & 0.27 & 0.45 \\ 
Rents from public housing & 13969 & 0.04 & 0.2 & 17455 & 0.03 & 0.18 \\ 
Monthly mortgage payments & 4394 & 1502.67 & 1160.26 & 6204 & 2096.53 & 1749.82 \\ 
Monthly rental payments & 3573 & 1050.52 & 565.1 & 5495 & 1490.23 & 838.43 \\ 
Employed full-time & 13969 & 0.42 & 0.49 & 17462 & 0.42 & 0.49 \\ 
Employed part-time & 13969 & 0.2 & 0.4 & 17462 & 0.21 & 0.41 \\ 
Neighbourhood decile of disadvantage & 13969 & 5.4 & 2.9 & 17448 & 5.6 & 2.87 \\ 
Eqv. household disposable income (\$1,000's) & 13969 & 42.44 & 29.82 & 17462 & 57.61 & 39.58 \\ 
Physical component summary & 12323 & 49.68 & 10.5 & 15698 & 49.16 & 10.69\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> ss_subgroups_both.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Summary Statisics - Matched Subgroups at t = -1}\label{tab.ss.subgroups.both}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\hline
\hline
Subgroup & \multicolumn{3}{c}{Renters - Control} & \multicolumn{3}{c}{Renters - Treat} & \multicolumn{3}{c}{Owners - Control} & \multicolumn{3}{c}{Owners - Treat}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 1043 & 43.78 & 11.8 & 466 & 42.74 & 12.4 & 881 & 45.44 & 10.86 & 264 & 44.44 & 11.4 \\ 
Employed full-time & 1043 & 0.31 & 0.46 & 466 & 0.33 & 0.47 & 881 & 0.39 & 0.49 & 264 & 0.51 & 0.5 \\ 
Employed part-time & 1043 & 0.25 & 0.43 & 466 & 0.25 & 0.43 & 881 & 0.31 & 0.46 & 264 & 0.23 & 0.42 \\ 
Neighbourhood decile of disadvantage & 1043 & 2.5 & 1.36 & 466 & 2.47 & 1.27 & 881 & 2.76 & 1.34 & 264 & 2.78 & 1.28 \\ 
Disposable income (\$1,000's) & 1043 & 37.56 & 17.88 & 466 & 36.98 & 15.28 & 881 & 45.15 & 22.97 & 264 & 47.16 & 21.93 \\ 
Physical component summary (lag) & 1043 & 50.05 & 10.26 & 466 & 48.94 & 10.88 & 881 & 50.55 & 10.13 & 264 & 49.38 & 9.93\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> ss_subgroups_own.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Owners Summary Statisics - Matched Subgroups at t = 0}\label{tab.ss.subgroups.own0}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\hline
\hline
Subgroup & \multicolumn{3}{c}{Low - Control} & \multicolumn{3}{c}{Low - Treat} & \multicolumn{3}{c}{High - Control} & \multicolumn{3}{c}{High - Treat}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 2681 & 46.52 & 11.02 & 790 & 47.54 & 11.08 & 930 & 43.97 & 11.29 & 314 & 43.11 & 11.39 \\ 
Employed full-time & 2746 & 0.41 & 0.49 & 820 & 0.41 & 0.49 & 947 & 0.4 & 0.49 & 326 & 0.46 & 0.5 \\ 
Employed part-time & 2746 & 0.27 & 0.44 & 820 & 0.19 & 0.39 & 947 & 0.27 & 0.44 & 326 & 0.25 & 0.43 \\ 
Moved in last 12 months & 2737 & 0.07 & 0.25 & 816 & 0.05 & 0.21 & 942 & 0.05 & 0.21 & 325 & 0.05 & 0.21 \\ 
Disposable income (\$1,000's) & 2746 & 49.62 & 34.32 & 820 & 47.97 & 58.36 & 947 & 42.88 & 26.44 & 326 & 44.53 & 22.94 \\ 
Physical component summary & 2681 & 49.24 & 10.61 & 790 & 47.39 & 11.2 & 930 & 47.53 & 11.59 & 314 & 47.48 & 11.26\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> ss_subgroups_own_sens.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Owners Summary Statisics - Matched Subgroups at t = 0}\label{tab.ss.subgroups.own0}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\hline
\hline
Subgroup & \multicolumn{3}{c}{Low - Control} & \multicolumn{3}{c}{Low - Treat} & \multicolumn{3}{c}{High - Control} & \multicolumn{3}{c}{High - Treat}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 2732 & 70.95 & 17.6 & 816 & 72.17 & 18.31 & 943 & 66.95 & 17.89 & 324 & 65.57 & 18.23 \\ 
Employed full-time & 2746 & 0.41 & 0.49 & 820 & 0.41 & 0.49 & 947 & 0.4 & 0.49 & 326 & 0.46 & 0.5 \\ 
Employed part-time & 2746 & 0.27 & 0.44 & 820 & 0.19 & 0.39 & 947 & 0.27 & 0.44 & 326 & 0.25 & 0.43 \\ 
Moved in last 12 months & 2737 & 0.07 & 0.25 & 816 & 0.05 & 0.21 & 942 & 0.05 & 0.21 & 325 & 0.05 & 0.21 \\ 
Disposable income (\$1,000's) & 2746 & 49.62 & 34.32 & 820 & 47.97 & 58.36 & 947 & 42.88 & 26.44 & 326 & 44.53 & 22.94 \\ 
Physical component summary & 2681 & 49.24 & 10.61 & 790 & 47.39 & 11.2 & 930 & 47.53 & 11.59 & 314 & 47.48 & 11.26\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> ss_subgroups_rent.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Summary Statisics - Matched Subgroups at t = -2}\label{tab.ss.subgroups.rent0}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\hline
\hline
Subgroup & \multicolumn{3}{c}{Renters - Control} & \multicolumn{3}{c}{Renters - Treat} & \multicolumn{3}{c}{Owners - Control} & \multicolumn{3}{c}{Owners - Treat}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 1043 & 43.78 & 11.8 & 466 & 42.74 & 12.4 & 881 & 45.44 & 10.86 & 264 & 44.44 & 11.4 \\ 
Employed full-time & 1043 & 0.31 & 0.46 & 466 & 0.33 & 0.47 & 881 & 0.39 & 0.49 & 264 & 0.51 & 0.5 \\ 
Employed part-time & 1043 & 0.25 & 0.43 & 466 & 0.25 & 0.43 & 881 & 0.31 & 0.46 & 264 & 0.23 & 0.42 \\ 
Neighbourhood decile of disadvantage & 1043 & 4.46 & 2.75 & 466 & 4.39 & 2.61 & 881 & 5.02 & 2.7 & 264 & 5.09 & 2.58 \\ 
Disposable income (\$1,000's) & 1043 & 37.56 & 17.88 & 466 & 36.98 & 15.28 & 881 & 45.15 & 22.97 & 264 & 47.16 & 21.93 \\ 
Physical component summary (lag) & 1043 & 50.05 & 10.26 & 466 & 48.94 & 10.88 & 881 & 50.55 & 10.13 & 264 & 49.38 & 9.93\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> ss_subgroups_rent_multi.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Renters Summary Statisics - Matched Subgroups at t = 0}\label{tab.ss.subgroups.own0}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\hline
\hline
Subgroup & \multicolumn{3}{c}{Low - Control} & \multicolumn{3}{c}{Low - Treat} & \multicolumn{3}{c}{High - Control} & \multicolumn{3}{c}{High - Treat}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 992 & 45.66 & 11.16 & 245 & 44.39 & 12.69 & 710 & 42.4 & 12.33 & 412 & 40.15 & 12.81 \\ 
Employed full-time & 1007 & 0.44 & 0.5 & 252 & 0.46 & 0.5 & 734 & 0.38 & 0.49 & 424 & 0.36 & 0.48 \\ 
Employed part-time & 1007 & 0.25 & 0.43 & 252 & 0.23 & 0.42 & 734 & 0.24 & 0.43 & 424 & 0.25 & 0.43 \\ 
Moved in last 12 months & 1002 & 0.3 & 0.46 & 248 & 0.25 & 0.44 & 733 & 0.33 & 0.47 & 422 & 0.3 & 0.46 \\ 
Disposable income (\$1,000's) & 1007 & 44.88 & 21.09 & 252 & 43.47 & 22.88 & 734 & 41.25 & 24.57 & 424 & 37.07 & 15.4 \\ 
Physical component summary & 992 & 50.5 & 10.26 & 245 & 51.12 & 10.31 & 710 & 50.24 & 10.37 & 412 & 48.49 & 11.25\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> ss_subgroups_rent_sens.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Renters Summary Statisics - Matched Subgroups at t = 0}\label{tab.ss.subgroups.own0}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrr}
\hline
\hline
Subgroup & \multicolumn{3}{c}{Low - Control} & \multicolumn{3}{c}{Low - Treat} & \multicolumn{3}{c}{High - Control} & \multicolumn{3}{c}{High - Treat}  \\ 
 Variable & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} \\ 
\hline
Mental component summary & 1003 & 69.37 & 18.23 & 252 & 67.8 & 19.5 & 728 & 64.88 & 19.57 & 424 & 62.31 & 20.88 \\ 
Employed full-time & 1007 & 0.44 & 0.5 & 252 & 0.46 & 0.5 & 734 & 0.38 & 0.49 & 424 & 0.36 & 0.48 \\ 
Employed part-time & 1007 & 0.25 & 0.43 & 252 & 0.23 & 0.42 & 734 & 0.24 & 0.43 & 424 & 0.25 & 0.43 \\ 
Moved in last 12 months & 1002 & 0.3 & 0.46 & 248 & 0.25 & 0.44 & 733 & 0.33 & 0.47 & 422 & 0.3 & 0.46 \\ 
Disposable income (\$1,000's) & 1007 & 44.88 & 21.09 & 252 & 43.47 & 22.88 & 734 & 41.25 & 24.57 & 424 & 37.07 & 15.4 \\ 
Physical component summary & 992 & 50.5 & 10.26 & 245 & 51.12 & 10.31 & 710 & 50.24 & 10.37 & 412 & 48.49 & 11.25\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> tab_baseline_fe.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Jun 18, 2021 - 6:31:01 PM
\begingroup 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & \multicolumn{4}{c}{ Mental Health (MCS)} \\ 
 & \multicolumn{2}{c}{Renters} & \multicolumn{2}{c}{Owners} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\\[-1.8ex] & FE1 & FE2 & FE1. & FE2.\\ 
\hline \\[-1.8ex] 
 missed\_house & $-$1.84$^{***}$ & $-$1.01$^{***}$ & $-$1.00$^{***}$ & $-$0.50$^{*}$ \\ 
  & (0.20) & (0.20) & (0.20) & (0.20) \\ 
  non\_house\_fh & $-$1.52$^{***}$ &  & $-$1.22$^{***}$ &  \\ 
  & (0.13) &  & (0.11) &  \\ 
  missed\_bills &  & $-$0.98$^{***}$ &  & $-$0.61$^{***}$ \\ 
  &  & (0.17) &  & (0.15) \\ 
  missed\_sold &  & $-$0.85$^{***}$ &  & $-$1.01$^{***}$ \\ 
  &  & (0.22) &  & (0.24) \\ 
  missed\_meals &  & $-$1.92$^{***}$ &  & $-$1.77$^{***}$ \\ 
  &  & (0.28) &  & (0.39) \\ 
  missed\_heat &  & $-$1.48$^{***}$ &  & $-$1.01$^{**}$ \\ 
  &  & (0.31) &  & (0.37) \\ 
  missed\_family &  & $-$0.64$^{***}$ &  & $-$0.82$^{***}$ \\ 
  &  & (0.15) &  & (0.15) \\ 
  missed\_community &  & $-$0.54$^{*}$ &  & $-$1.15$^{***}$ \\ 
  &  & (0.25) &  & (0.35) \\ 
  missed\_emergency &  & $-$0.98$^{***}$ &  & $-$0.91$^{***}$ \\ 
  &  & (0.17) &  & (0.19) \\ 
  linc\_disp\_eqv & 0.13 & 0.07 & 0.45$^{***}$ & 0.42$^{***}$ \\ 
  & (0.12) & (0.12) & (0.11) & (0.11) \\ 
  emp\_full & 1.34$^{***}$ & 1.17$^{***}$ & 0.77$^{***}$ & 0.72$^{***}$ \\ 
  & (0.20) & (0.20) & (0.16) & (0.16) \\ 
  emp\_part & 1.17$^{***}$ & 1.07$^{***}$ & 0.80$^{***}$ & 0.77$^{***}$ \\ 
  & (0.19) & (0.19) & (0.15) & (0.15) \\ 
  lag\_pcs & 0.04$^{***}$ & 0.04$^{***}$ & 0.02$^{***}$ & 0.02$^{***}$ \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) \\ 
  factor(neighbourhood)2 & $-$0.03 & $-$0.04 & 0.32 & 0.36 \\ 
  & (0.31) & (0.31) & (0.45) & (0.45) \\ 
  factor(neighbourhood)3 & 0.46 & 0.48 & 0.84 & 0.88$^{*}$ \\ 
  & (0.32) & (0.32) & (0.43) & (0.43) \\ 
  factor(neighbourhood)4 & $-$0.31 & $-$0.39 & 0.19 & 0.17 \\ 
  & (0.34) & (0.33) & (0.46) & (0.46) \\ 
  factor(neighbourhood)5 & $-$0.15 & $-$0.18 & 0.21 & 0.22 \\ 
  & (0.32) & (0.32) & (0.42) & (0.42) \\ 
  factor(neighbourhood)6 & $-$0.20 & $-$0.23 & 0.41 & 0.43 \\ 
  & (0.34) & (0.34) & (0.44) & (0.43) \\ 
  factor(neighbourhood)7 & $-$0.0001 & $-$0.07 & $-$0.13 & $-$0.11 \\ 
  & (0.34) & (0.34) & (0.43) & (0.43) \\ 
  factor(neighbourhood)8 & 0.18 & 0.12 & $-$0.06 & $-$0.07 \\ 
  & (0.35) & (0.34) & (0.44) & (0.44) \\ 
  factor(neighbourhood)9 & 0.20 & 0.15 & 0.41 & 0.42 \\ 
  & (0.35) & (0.35) & (0.46) & (0.46) \\ 
  factor(neighbourhood)10 & 0.13 & 0.07 & $-$0.06 & $-$0.06 \\ 
  & (0.39) & (0.39) & (0.45) & (0.45) \\ 
 \hline \\[-1.8ex] 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 
\endgroup 


==> tab_baseline_fe3040_dyn.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Jun 04, 2021 - 12:02:37 PM
\begin{table}[!htbp] \centering 
  \caption{Fixed effects results using 30/40 rule} 
  \label{tab.mcs.fe.baseline} 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{Dependent variable: Mental health summary (MCS)} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{ .................. Renters .................. .................. Owners .................. } \\ 
 & FE & FE+ctls & Dynamics & FE & FE+ctls & Dynamics \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 Stress, 30/40 Rule & $-$0.51$^{***}$ & $-$0.32$^{*}$ & $-$0.32$^{*}$ & $-$0.47$^{***}$ & $-$0.26$^{*}$ & $-$0.34$^{*}$ \\ 
  & (0.12) & (0.13) & (0.15) & (0.13) & (0.13) & (0.14) \\ 
  Financial Hardship & $-$2.09$^{***}$ & $-$2.03$^{***}$ & $-$1.94$^{***}$ & $-$1.61$^{***}$ & $-$1.62$^{***}$ & $-$1.53$^{***}$ \\ 
  & (0.11) & (0.11) & (0.13) & (0.10) & (0.10) & (0.11) \\ 
  Lag Stress, 30/40 Rule &  &  & 0.25 &  &  & $-$0.12 \\ 
  &  &  & (0.14) &  &  & (0.15) \\ 
  Lag Financial Hardship &  &  & $-$0.43$^{***}$ &  &  & $-$0.47$^{***}$ \\ 
  &  &  & (0.12) &  &  & (0.10) \\ 
 \hline \\[-1.8ex] 
Controls & No & Yes & Yes & No & Yes & Yes \\ 
Year Dummies & Yes & Yes & Yes & Yes & Yes & Yes \\ 
Observations & 54393 & 54393 & 39776 & 84619 & 84619 & 67827 \\ 
F Statistic & 183.5 & 178.36 & 4.38 & 133.57 & 138.91 & 2.977 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{7}{l}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\multicolumn{7}{l}{F Statistic null: financial hardship and housing stress are jointly zero,} \\ 
\multicolumn{7}{l}{or housing stress and its first lag are jointly zero.} \\ 
\multicolumn{7}{l}{Controls: Moved last 12 months, eqv. household disposable income, employment status,} \\ 
\multicolumn{7}{l}{and their first lag for the dynamic model.} \\ 
\multicolumn{7}{l}{In this model, housing stress has an additive effect as } \\ 
\end{tabular} 
\end{table} 


==> tab_baseline_fe_dyn.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Jun 04, 2021 - 11:59:32 AM
\begin{table}[!htbp] \centering 
  \caption{Baseline fixed effects results} 
  \label{tab.mcs.fe.baseline} 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{Dependent variable: Mental health summary (MCS)} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{ .................... Renters .................... .................... Owners .................... } \\ 
 & FE & FE+ctls & Dynamics & FE & FE+ctls & Dynamics \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 Housing Stress & $-$1.51$^{***}$ & $-$1.45$^{***}$ & $-$1.50$^{***}$ & $-$0.71$^{***}$ & $-$0.67$^{***}$ & $-$0.60$^{**}$ \\ 
  & (0.17) & (0.17) & (0.20) & (0.19) & (0.18) & (0.21) \\ 
  Financial Hardship & $-$1.74$^{***}$ & $-$1.68$^{***}$ & $-$1.58$^{***}$ & $-$1.47$^{***}$ & $-$1.48$^{***}$ & $-$1.39$^{***}$ \\ 
  & (0.12) & (0.11) & (0.13) & (0.11) & (0.10) & (0.12) \\ 
  Lag Housing Stress &  &  & $-$0.005 &  &  & $-$0.51$^{**}$ \\ 
  &  &  & (0.19) &  &  & (0.19) \\ 
  Lag Financial Hardship &  &  & $-$0.38$^{**}$ &  &  & $-$0.35$^{***}$ \\ 
  &  &  & (0.13) &  &  & (0.11) \\ 
 \hline \\[-1.8ex] 
Controls & No & Yes & Yes & No & Yes & Yes \\ 
Year Dummies & Yes & Yes & Yes & Yes & Yes & Yes \\ 
Observations & 54393 & 54393 & 39776 & 84619 & 84619 & 67827 \\ 
F Statistic & 210.49 & 208.1 & 30.12 & 134.36 & 140.24 & 6.66 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{7}{l}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\multicolumn{7}{l}{F Statistic null: financial hardship and housing stress are jointly zero,} \\ 
\multicolumn{7}{l}{or housing stress and its first lag are jointly zero.} \\ 
\multicolumn{7}{l}{Controls: Moved last 12 months, eqv. household disposable income, employment status,} \\ 
\multicolumn{7}{l}{and their first lag for the dynamic model.} \\ 
\end{tabular} 
\end{table} 


==> tab_baseline_fe_full.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Jun 12, 2021 - 3:21:16 PM
\begingroup 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & \multicolumn{4}{c}{ Mental Health (MCS)} \\ 
 & \multicolumn{2}{c}{Renters} & \multicolumn{2}{c}{Owners} \\ 
\\[-1.8ex] & .Pooled & FE & Pooled & FE.\\ 
\hline \\[-1.8ex] 
 Housing Financial Hardship & $-$2.10$^{***}$ & $-$1.45$^{***}$ & $-$0.89$^{***}$ & $-$0.50$^{**}$ \\ 
  & (0.23) & (0.17) & (0.25) & (0.16) \\ 
  Non-housing Financial Hardship & $-$5.06$^{***}$ & $-$1.68$^{***}$ & $-$5.47$^{***}$ & $-$1.64$^{***}$ \\ 
  & (0.16) & (0.11) & (0.14) & (0.09) \\ 
  Moved last 12 months & $-$0.33$^{**}$ & $-$0.12 & $-$0.70$^{***}$ & 0.15$^{*}$ \\ 
  & (0.11) & (0.09) & (0.09) & (0.07) \\ 
  Disposable income & 0.01$^{**}$ & 0.01$^{**}$ & 0.01$^{***}$ & 0.004$^{***}$ \\ 
  & (0.003) & (0.002) & (0.001) & (0.001) \\ 
  Employed full-time & 3.76$^{***}$ & 1.88$^{***}$ & 1.05$^{***}$ & 0.52$^{***}$ \\ 
  & (0.20) & (0.18) & (0.13) & (0.10) \\ 
  Employed part-time & 2.54$^{***}$ & 1.55$^{***}$ & 0.54$^{***}$ & 0.61$^{***}$ \\ 
  & (0.21) & (0.17) & (0.13) & (0.09) \\ 
  Physical component summary & $-$0.14$^{***}$ & $-$0.35$^{***}$ & $-$0.06$^{***}$ & $-$0.25$^{***}$ \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) \\ 
 \hline \\[-1.8ex] 
Controls & Yes & Yes & Yes & Yes \\ 
Year dummies & Yes & Yes & Yes & Yes \\ 
Individuals & 13644 & 13644 & 22581 & 22581 \\ 
Degrees of freedom & 54367 & 40724 & 168581 & 146001 \\ 
R-Squared & 0.102 & 0.096 & 0.047 & 0.057 \\ 
F-Statistic & 717.39 & 208.1 & 873.01 & 228.6 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 
\endgroup 


==> tab_did_full.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Jun 08, 2021 - 3:02:20 PM
\begingroup 
\normalsize 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{Dependent Variable: Mental Health (MCS)} \\ 
\cline{2-5} 
\\[-1.8ex] & \multicolumn{4}{c}{........... Renters ........... ........... Owners ...........} \\ 
 & Low & High & Low & High \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Treat:1[t=0] & $-$1.40 & $-$1.94$^{**}$ & $-$0.01 & $-$0.32 \\ 
  & (0.81) & (0.74) & (0.42) & (0.71) \\ 
  Treat:1[t=-1] & $-$0.05 & 0.02 & $-$0.04 & 0.23 \\ 
  & (0.71) & (0.70) & (0.39) & (0.70) \\ 
  Treat & 0.04 & $-$0.48 & 0.98$^{*}$ & $-$0.82 \\ 
  & (0.70) & (0.73) & (0.40) & (0.71) \\ 
  1[t=-1] & $-$0.80$^{**}$ & $-$0.40 & $-$0.49$^{**}$ & $-$0.08 \\ 
  & (0.31) & (0.40) & (0.18) & (0.35) \\ 
  1[t=0] & $-$1.81$^{***}$ & $-$0.46 & $-$1.67$^{***}$ & $-$0.62 \\ 
  & (0.34) & (0.43) & (0.21) & (0.38) \\ 
  Employed FT & 3.56$^{***}$ & 4.37$^{***}$ & 2.52$^{***}$ & 4.42$^{***}$ \\ 
  & (0.62) & (0.69) & (0.36) & (0.66) \\ 
  Employed PT & 2.50$^{***}$ & 3.46$^{***}$ & 1.65$^{***}$ & 3.00$^{***}$ \\ 
  & (0.64) & (0.71) & (0.37) & (0.68) \\ 
  Income & $-$0.02 & 0.002 & 0.003 & $-$0.01 \\ 
  & (0.01) & (0.01) & (0.004) & (0.01) \\ 
  Moved & 0.75 & 0.97$^{*}$ & $-$0.25 & $-$1.67$^{*}$ \\ 
  & (0.40) & (0.48) & (0.45) & (0.70) \\ 
  PCS & $-$0.14$^{***}$ & $-$0.13$^{***}$ & $-$0.09$^{***}$ & $-$0.03 \\ 
  & (0.03) & (0.03) & (0.02) & (0.02) \\ 
  Intercept & 53.07$^{***}$ & 46.71$^{***}$ & 51.14$^{***}$ & 43.95$^{***}$ \\ 
  & (1.60) & (1.55) & (0.79) & (1.24) \\ 
 \hline \\[-1.8ex] 
Individuals & 1259 & 1158 & 3566 & 1273 \\ 
Observations & 3663 & 3369 & 10313 & 3699 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 
\endgroup 


==> tab_did_full2.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Jun 25, 2021 - 5:48:25 PM
\begingroup 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{Mental Component Summary} \\ 
 & Renters & Owners \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 Treat:1[t=0] & $-$2.05$^{*}$ & $-$0.96 \\ 
  & (0.87) & (0.94) \\ 
  Treat:1[t=-1] & 0.13 & $-$0.21 \\ 
  & (0.84) & (0.95) \\ 
  Treat & $-$1.14 & $-$0.59 \\ 
  & (0.86) & (0.96) \\ 
  1[t=-1] & $-$0.78 & $-$0.15 \\ 
  & (0.53) & (0.52) \\ 
  1[t=0] & $-$0.96 & $-$0.74 \\ 
  & (0.55) & (0.54) \\ 
  Disposable income & $-$0.10 & $-$0.06 \\ 
  & (0.48) & (0.57) \\ 
  Employed full-time & 2.77$^{***}$ & 2.95$^{***}$ \\ 
  & (0.61) & (0.73) \\ 
  Employed part-time & 2.18$^{***}$ & 2.15$^{**}$ \\ 
  & (0.62) & (0.74) \\ 
  Physical component summary & 0.06$^{*}$ & 0.07$^{*}$ \\ 
  & (0.03) & (0.03) \\ 
  Neighbourhood (Q2) & 1.66$^{*}$ & $-$0.76 \\ 
  & (0.65) & (0.81) \\ 
  Neighbourhood (Q3) & $-$0.07 & $-$1.10 \\ 
  & (0.77) & (0.87) \\ 
  Neighbourhood (Q4) & $-$0.31 & $-$1.17 \\ 
  & (0.86) & (0.92) \\ 
  Neighbourhood (Q5) & $-$0.03 & $-$0.45 \\ 
  & (0.92) & (0.92) \\ 
 \hline \\[-1.8ex] 
Calendar Year Fixed Effects & Yes & Yes \\ 
Individuals & 1552 & 1183 \\ 
Observations & 3748 & 2869 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{3}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 
\endgroup 


==> tab_did_full_sens.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Jun 08, 2021 - 4:13:00 PM
\begingroup 
\normalsize 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{Dependent Variable: Mental Health (MCS)} \\ 
\cline{2-5} 
\\[-1.8ex] & \multicolumn{4}{c}{........... Renters ........... ........... Owners ...........} \\ 
 & Low & High & Low & High \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Treat:1[t=0] & $-$2.08 & $-$2.69$^{*}$ & $-$0.05 & $-$1.39 \\ 
  & (1.31) & (1.16) & (0.69) & (1.12) \\ 
  Treat:1[t=-1] & 0.57 & $-$0.58 & 0.24 & $-$0.34 \\ 
  & (1.10) & (1.11) & (0.62) & (1.15) \\ 
  Treat & $-$0.02 & 0.32 & 1.53$^{*}$ & $-$0.34 \\ 
  & (1.16) & (1.18) & (0.67) & (1.20) \\ 
  1[t=-1] & $-$1.41$^{**}$ & 0.06 & $-$0.78$^{**}$ & $-$0.16 \\ 
  & (0.50) & (0.64) & (0.29) & (0.57) \\ 
  1[t=0] & $-$3.11$^{***}$ & $-$0.49 & $-$2.47$^{***}$ & $-$0.80 \\ 
  & (0.56) & (0.67) & (0.32) & (0.60) \\ 
  Employed FT & 5.55$^{***}$ & 6.49$^{***}$ & 3.32$^{***}$ & 5.89$^{***}$ \\ 
  & (1.02) & (1.12) & (0.59) & (1.04) \\ 
  Employed PT & 3.59$^{***}$ & 5.19$^{***}$ & 2.15$^{***}$ & 4.00$^{***}$ \\ 
  & (1.05) & (1.13) & (0.60) & (1.08) \\ 
  Income & $-$0.03 & 0.01 & 0.01 & 0.002 \\ 
  & (0.02) & (0.02) & (0.01) & (0.01) \\ 
  Moved & 0.95 & 1.37 & $-$0.37 & $-$2.32$^{*}$ \\ 
  & (0.66) & (0.78) & (0.70) & (1.12) \\ 
  PCS & $-$0.02 & 0.02 & 0.01 & 0.12$^{**}$ \\ 
  & (0.05) & (0.05) & (0.02) & (0.04) \\ 
  Intercept & 71.36$^{***}$ & 59.65$^{***}$ & 70.65$^{***}$ & 58.49$^{***}$ \\ 
  & (2.60) & (2.65) & (1.25) & (2.04) \\ 
 \hline \\[-1.8ex] 
Individuals & 1259 & 1158 & 3566 & 1273 \\ 
Observations & 3663 & 3369 & 10313 & 3699 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{5}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\end{tabular} 
\endgroup 


==> tab_sf36mh_fe_dyn.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Jun 04, 2021 - 12:01:05 PM
\begin{table}[!htbp] \centering 
  \caption{Robustness - Mental health scale dependent variable} 
  \label{tab.sf36mh.fe.baseline} 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{Dependent variable: mental health scale} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{ .................. Renters .................. .................. Owners .................. } \\ 
 & FE & FE+ctls & Dynamics & FE & FE+ctls & Dynamics \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 Housing Stress & $-$2.27$^{***}$ & $-$2.20$^{***}$ & $-$2.27$^{***}$ & $-$1.25$^{***}$ & $-$1.18$^{***}$ & $-$1.02$^{**}$ \\ 
  & (0.27) & (0.26) & (0.31) & (0.30) & (0.29) & (0.33) \\ 
  Financial Hardship & $-$2.49$^{***}$ & $-$2.34$^{***}$ & $-$2.32$^{***}$ & $-$2.35$^{***}$ & $-$2.33$^{***}$ & $-$2.23$^{***}$ \\ 
  & (0.19) & (0.18) & (0.21) & (0.17) & (0.17) & (0.19) \\ 
  Lag Housing Stress &  &  & 0.14 &  &  & $-$0.85$^{**}$ \\ 
  &  &  & (0.30) &  &  & (0.31) \\ 
  Lag Financial Hardship &  &  & $-$0.42$^{*}$ &  &  & $-$0.51$^{**}$ \\ 
  &  &  & (0.21) &  &  & (0.17) \\ 
 \hline \\[-1.8ex] 
Controls & No & Yes & Yes & No & Yes & Yes \\ 
Year Dummies & Yes & Yes & Yes & Yes & Yes & Yes \\ 
Observations & 54393 & 54393 & 39776 & 84619 & 84619 & 67827 \\ 
F Statistic & 175.26 & 160.71 & 28.28 & 140.49 & 137.62 & 7.49 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{7}{l}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
\multicolumn{7}{l}{F Statistic null: financial hardship and housing stress are jointly zero,} \\ 
\multicolumn{7}{l}{or housing stress and its first lag are jointly zero.} \\ 
\multicolumn{7}{l}{Controls: Moved last 12 months, eqv. household disposable income, employment status,} \\ 
\multicolumn{7}{l}{and their first lag for the dynamic model.} \\ 
\end{tabular} 
\end{table} 

